Robust Anomaly Detection in Dynamic Networks

We propose two robust methods for anomaly detection in dynamic networks in which the properties of normal traffic are time-varying. We formulate the robust anomaly detection problem as a binary composite hypothesis testing problem and propose two methods: a model-free and a model-based one, leveraging techniques from the theory of large deviations. Both methods require a family of Probability Laws (PLs) that represent normal properties of traffic. We devise a two-step procedure to estimate this family of PLs. We compare the performance of our robust methods and their vanilla counterparts, which assume that normal traffic is stationary, on a network with a diurnal normal pattern and a common anomaly related to data exfiltration. Simulation results show that our robust methods perform better than their vanilla counterparts in dynamic networks.

==> GreedySolve.tex <==
\begin{algorithmic}
\Function {GreedySetCover}{$\bA$, $\gamma$, $\bc_v$}
    \State\textbf{Init}: $\bx^0 \gets \bzero$, $C \gets \varnothing$
    \While {|C| < M}
    % \For {$j \mbox{ such that }\bx[j] = 0$}
    % \State $\bs[j] \gets \frac{\sum_{i\notin C} a_{ij}}{1 + \gamma \bc_v[j]} $
    % \EndFor
    % \State $j^+ \gets \arg\max_{j:\bx[j]=0} \bs[j]$
    \State $j^+ \gets \arg\max_{j:\bx[j]=0} \frac{\sum_{i\notin C} a_{ij}}{1 + \gamma \bc_v[j]} $
    \State $\bx[j^+] = 1$, $C = C \cup \{i : a_{ij^+} = 1\}$
    \EndWhile
    \State \Return $\bx$
    % \State \Return $\bx$, $\mathbf{1}^T \bx + \gamma \bc_v^T \bx$
\EndFunction

\end{algorithmic}


==> LocalSearch.tex <==
\begin{algorithmic}
\Function {LocalSearch}{$\bx$, $\bA$}
    \ForAll {$j \in \{i: x[i] > 0\}$}
        \State $\bx[j] \gets 0$
        \If {$\texttt{Satisfy}(\bx, \bA[j]) = \mbox{True}$}
            \State \Return $\bx$
        \EndIf
        \State $\bx[j] \gets 1$
    \EndFor
    \State \Return $\bx$
\EndFunction
\end{algorithmic}


==> model_selection.tex <==
\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\Continue}{\textbf{continue}}
\newcommand{\Break}{\State \algorithmicbreak}
\begin{algorithmic}
    \Function {RefinePl}{D, $\lambda$}
    \State\textbf{Init}: $\bx^0 \gets \bzero$, $\bA \gets \bzero$
    \For {$k = 1 \to n$}
    % \State Check whether ${\bx^k}$ Satisfis constaints.
    \State {$\bx^k \gets \bx^{k-1}$}
    % \If {$\bx^{k-1} \notin \scrF_k $}
    \If {$\texttt{Satisfy}(\bx^{k}, k) = \mbox{True}$}
        \State \Continue
    \EndIf
        % \State $\bc_k = $
        \ForAll {$i \in \{i: D_{ik} < \lambda\}$}
            \State $\bx^k[i] \gets 1$ 
            \Comment Get a Feasible Solution
            \State $\bA[i] \gets k$ 
            \State {$\bx^{k} \gets \texttt{LocalSearch}(\bx^k, \bA, k)$ }
            % \If {$\bx^+$ is better then $\bx$}
            %     \State {$\bx_k \gets \bx^+$}
            %     \Break
            % \EndIf

        \EndFor
    % \EndIf
    \EndFor
    \EndFunction

    % \Function {LocalSearch}{$\bx$, $\scrF$}
    %     \ForAll {$j \in \{i: x[i] > 0\}$}
    %         \State $\bx[j] \gets 0$
    %         \If {$\bx \in \scrF$}
    %             \State \Return $\bx$
    %         \EndIf
    %         \State $\bx[j] \gets 1$
    %     \EndFor
    %     \Return $\bx$
    % \EndFunction

% \If {$i\geq maxval$}
%     \State $i\gets 0$
% \Else
%     \If {$i+k\leq maxval$}
%         \State $i\gets i+k$
%     \EndIf
% \EndIf
\end{algorithmic}


==> mymacros_2cln_ieee.tex <==
% Equations ... 
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\newcommand{\benon}{\begin{equation*}}  
%\newcommand{\ee}{\end{equation}}
%\newcommand{\eenon}{\end{equation*}}
\newcommand{\bemuln}[1]{\begin{multline}\label{#1}}
\newcommand{\bemul}{\begin{multline*}}
%\newcommand{\emuln}{\end{multline}}
%\newcommand{\emul}{\end{multline*}}
\newcommand{\bee}{\begin{eqnarray*}}
\newcommand{\eee}{\end{eqnarray*}}
\newcommand{\been}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eeen}{\end{eqnarray}}
\newcommand{\began}[1]{\begin{gather}\label{#1}}
\newcommand{\bega}{\begin{gather*}}
%\newcommand{\egan}{\end{gather}}
%\newcommand{\ega}{\end{gather*}}
\newcommand{\bealn}[1]{\begin{align}\label{#1}}
\newcommand{\beal}{\begin{align*}}
%\newcommand{\ealn}{\end{align}}
%\newcommand{\eal}{\end{align*}}
\newcommand{\bealatn}[2]{\begin{alignat}{#1}\label{#2}}
\newcommand{\bealat}{\begin{alignat*}}
%\newcommand{\ealatn}{\end{alignat}}
%\newcommand{\ealat}{\end{alignat*}}
\newcommand{\bexalatn}[1]{\begin{xalignat}\label{#1}}
\newcommand{\bexalat}{\begin{xalignat*}}
%\newcommand{\exalatn}{\end{xalignat}}
%\newcommand{\exalat}{\end{xalignat*}}


% Various...
%\newcommand{\qed}{\newline \mbox{ } \hfill 
%            \rule[-1pt]{2.5mm}{2.5mm}\par\vskip 10pt }
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\pf}{\vskip 5 pt \noindent {\bf{Proof: }}}
\newcommand{\disc}{\vskip 5 pt \noindent {\bf Discussion: }}
\newcommand{\mot}{\vskip 5 pt \noindent {\bf Motivation: }}
%\newcommand{\note}{\vskip 5 pt \noindent {\bf Note: }}
\newcommand{\rems}{\vskip 5 pt \noindent {\bf Remarks: }}
\newcommand{\rem}{\vskip 5 pt \noindent {\bf Remark: }}
%\newcommand{\Nt}{{\tilde N}}
\newcommand{\diag}{\text{diag}}
\newcommand{\tsum}{\textstyle\sum}
\newcommand{\dsum}{\displaystyle\sum}
\newcommand{\tprod}{\textstyle\prod}
\newcommand{\dprod}{\displaystyle\prod}
\def\argmax{\mathop{\rm arg\,max}}

%Font commands
\newcommand{\mb}{\mathbf}
\newcommand{\bsy}{\boldsymbol}
\newcommand{\mn}{\mathnormal}
\newcommand{\mbb}{\mathbb}
\newcommand{\bosy}{\boldsymbol}


% Theorems ...
% \theoremstyle{plain} 
% \newtheorem{thm}{Theorem}[section]
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
%\theoremstyle{definition} 
%\theorembodyfont{\it}
\newtheorem{defi}{Definition}
\newtheorem{ass}{Assumption}
\newtheorem{algo}{Algorithm} 
\newtheorem{cond}{Condition}
\renewcommand{\theass}{\Alph{ass}} 




